Model-Based Event Detection in Wireless Sensor Networks

In this paper we present an application of techniques from statistical signal processing to the problem of event detection in wireless sensor networks used for environmental monitoring. The proposed approach uses the well-established Principal Component Analysis (PCA) technique to build a compact model of the observed phenomena that is able to capture daily and seasonal trends in the collected measurements. We then use the divergence between actual measurements and model predictions to detect the existence of discrete events within the collected data streams. Our preliminary results show that this event detection mechanism is sensitive enough to detect the onset of rain events using the temperature modality of a wireless sensor network.

==> etc.tex <==
There are two variants to the problem of \emph{event detection}. In
the first case, motes in the network detect the events as they happen
and collectively change their behavior to react to these
changes. Adaptation strategies include changes in the sampling rate as
well as waking up other nodes in the network to increase spatial
coverage of the detected event~\cite{DGA+05,GS04}. In the offline
case, event detection happens at the database that stores the
measurements collected by the network and is used to automatically
identify 'interesting' regions within the swaths of data acquired by
the sensor network. 


\jg{
I think it might be better if we talk about the benefits of 
detecting events rather than referring the 2 variants. In some sense this 
exposes the fact that we havent done anything on the motes.
}


Also, the same model can be used for both online and offline applications, 
which means that the events detected in network are exactly same set of events 
reported by a model-based query interface.  Equivalently, the process of 
in-network adaptation does not change query results when compared with 
continuous sampling. If the system does not detect the event in-network, 
it would not be reported by the model-based query.
{\bf Alex: I do not see why this is an issue. Off-line we can alway do 
much fancier stuff. I would just leave this out entirely.}.

Finally, PCA is not inherently adaptive or dynamic; even though 
there are adaptive and dynamic versions of PCA \cite{}.
Therefore, PCA models cannot easily be built or updated in the sensor
network. {\bf alex: this is not true... those are quite simple. We just did not have time to try.
Tamas B. has written such a packge -- it is 50 lines of code}. 

We note that this is different from evaluating a pre-built model,
which may be done at motes.  Also, while our precision and recall values
are good from a information retrieval standpoint.  Significant
ambiguities persist in which events and non-events cannot be differentiated
based on their component loadings.  Perhaps more dynamic learning techniques,
{\em e.g.}~Bayesian networks \cite{} or hidden-Markov models \cite{} 
might better describe environmental behavior.


